Do Concept Bottleneck Models Learn as Intended?

Concept bottleneck models map from raw inputs to concepts, and then from concepts to targets. Such models aim to incorporate pre-specified, high-level concepts into the learning procedure, and have been motivated to meet three desiderata: interpretability, predictability, and intervenability. However, we find that concept bottleneck models struggle to meet these goals. Using post hoc interpretability methods, we demonstrate that concepts do not correspond to anything semantically meaningful in input space, thus calling into question the usefulness of concept bottleneck models in their current form.

==> regularize.tex <==
\section{Regularizing the New Concepts}
When learning the learned concepts, we may desire that the new concepts are independent of the specified concepts or are sufficiently diverse. We now discuss various desirable properties between the first $k$ dimensions of $\*z$ and the rest of the $h-k$ newly discovered concepts. We translate each property into regularizer to enforce via $\mathcal{L}_r$. 

\subsection{Minimizing Mutual Information}
A natural approach to enforcing diversity between the old concepts, $\*z_{:k}$, and new concepts, $\*z_{k:}$, is minimize the mutual information between the two. We want our new concepts not to contain redundant information from the old ones but to extract relevant information to the targets from the inputs. We propose the following loss function accordingly:
\begin{equation}
\begin{aligned}
    \mathcal{L}_r^{MI} = I(\*z_{:k}, \*z_{k:}) &= \int p(\*z) \log \frac{p(\*z)}{p(\*z_{:k})](\*z_{k:})} d\*z \\
    &= H(\*z_{:k}) + H(\*z_{k:}) - H(\*z)
\end{aligned}
\label{mi}
\end{equation}
where the distributions are obtained by integrating over the data:
\begin{equation}
    p(\*z) = \int p(\*z, \*x) d\*x.
\end{equation}
In practice this integral is approximated using samples from the training set. 
Unfortunately, estimating the distributions $p(\*z)$, $p(\*z_{:k})$ and $p(\*z_{k:})$ using samples from the training set is difficult due to the large number of concepts typically used. However, we can use distribution-free approaches to calculating MI. 
\citet{mine} propose one such approach to estimating mutual information via a \textit{neural information measure}, $I_{\Theta}(\mathcal{X},\mathcal{Z})$: this quantity is grounded in the dual representation of the Kullback-Leibler divergence between the joint and product of the marginals introduced in \cite{donsker}, which is parameterized by $\theta \in \Theta$ from a \textit{statistics network} $T_\Theta: \mathcal{X} \times \mathcal{Z} \rightarrow \mathbb{R}$: a deep neural network used to estimate the neural information measure from empirical samples from the joint ($\mathbb{P}_{\mathcal{X} \mathcal{Z}}$) and the product of the marginal distributions ($\mathbb{P}_{\mathcal{X}} \otimes \mathbb{P}_{\mathcal{Z}}$). The empirical neural information measure ($\widehat I$) is defined as follows by \citet{mine}:
\begin{equation}
\widehat I(\mathcal{X},\mathcal{Z}) = \sup_{\theta \in \Theta} \mathbb{E}_{\mathbb{P}_{\mathcal{X} \mathcal{Z}}}[T_\theta] - \log(\mathbb{E}_{\mathbb{P}_{\mathcal{X}}{ \otimes \mathbb{P}_\mathcal{Z}}}[e^{T_\theta}])
\end{equation}
We will use this approximation to calculate $I(\*z_{:k}, \*z_{k:})$ from the empirical samples of the extended concept bottleneck during training. Note we will have to train a MINE network at every epoch of training our extended CBM.

Another pragmatic alternative is to minimize the summation of the pairwise mutual information between each concept:
\begin{equation}
    \sum_{i=1}^h \sum_{j\neq i} I(z_i, z_j) = \sum_{i=1}^h \sum_{j\neq i} H(z_i) + H(z_j) - H(z_i, z_j).
\end{equation}
This requires estimating the pairwise distributions $p(z_i, z_j)$ and marginals $p(z_i)$ and $p(z_j)$, which is feasible. However, the number of pairwise mutual information to evaluate grows is $\frac{d(d-1)}{2}$, which can become overwhelming for large $d$. An additional simplification is to consider only the pairwise mutual informations between each new concept:
\begin{equation}
    \sum_{i=k+1}^d \sum_{j=k+1, j\neq i}^d I(z_i, z_j)
\end{equation}
which ensures diversity amongst the newly learned concepts.



% \subsection{Manipulating Adversarial}
% Adversary cannot predict $\*z_{k:}$ from $\*z_{:k}$. Similar to~\citep{madras2018learning}... 


\subsection{Enforcing Orthogonality}
We may wish to promote diversity amongst the latent variables, which can be achieved by including a regularization term in the loss:
$\sum_{n=1}^N \mathcal{L}_{r}(\*z_n)$.
There are a plethora of ways this can be achieved, most of which hinge upon the idea of \textit{angular diversification}. Suppose we have a vector representation, $\*a_i$, for each latent variable $z_i$. A natural approach to diversifying these representations is to ensure they are evenly spread out to different directions in space. For example, we could define the regularisation term to be
\begin{equation}
\small
\begin{aligned}
    \mathcal{L}_r^{AD}&(\*z_n) = \frac{1}{h(h-1)}\sum_{i=1}^h\sum_{j\neq i}^h \theta_{ij} \\
    &-  \frac{\alpha}{d(d-1)}\sum_{i=1}^h\sum_{j\neq i}^h \left(\theta_{ij} - \frac{1}{d(d-1)} \sum_{p=1}^d\sum_{q\neq p}^d \theta_{pq}\right)^2
\end{aligned}
\end{equation}
where 
\begin{align}
    \theta_{ij} = \operatorname{arccos}\left(\frac{\*a_{i}^T\*a_{j}}{\|\*a_{i}\|_2\|\*a_{j}\|_2}\right)
\end{align}
is the non-obtuse angle measuring the dissimilarity between vector representations of $z_{i}$ and $z_{j}$, $\*a_{i}$ and $\*a_{j}$. Alternatively, we could minimize the hyperspherical energy of the vector representations $\{\*a_i\}_{i=1}^d$, or enforce orthogonality. 

Regardless of the choice of regularization, these approaches demand access to a vector representation for each latent variable. 
One possible choice for the vector representation is the set of weights (and bias) used to obtain the latent variable. It is important to note that linearly independent weights do not correspond to independent latent variables---this also depends on the independence of the activations at the previous hidden layer. \emph{This observation suggests that applying angular regularisation to the weights at every layer may be appropriate.}

Another method for obtaining a vector representation of each concept would be as follows. Let $\*z_{ni} \in \mathbb{R}^M$ correspond to a set of $M$ values in the intermediate layer for concept $i$. We obtain the prediction for concept $i$ by linearly projecting $\*z_{ni}$ onto a single-dimension:
\begin{equation}
    \hat{c}_{ni} = \*\beta^T \*z_{ni} + b
\end{equation}
where $\*\beta \in \mathbb{R}^M$ and $b\in \mathbb{R}$ are the parameters of the projection, which are the same for all concepts. A drawback of this approach is that it requires the use of a $M \times k$-dimension intermediate layer, which could be too large for large concepts. \todor{This approach widens the bottleneck without the addition of any new concepts...}



% \section{Probabilistic Modelling Perspective}
% Instead of taking a deterministic approach to diversifying the $k$ specified concepts from the $h-k$ learned concepts, we can consider thinking about CBMs in a probabilistic manner.
% If we use a factorised prior $p(\*z)$, such as an isotropic Gaussian, will encourage the posterior $p(\*z | \*x)$ to also be factorised (i.e. independence $p(\*z | \*x) \approx p(\*z_1 | \*x)\ldots p(\*z_h | \*x)$). We can place a prior distribution over the latent variables if we assume the generative model
% \begin{equation}
%     p(\*x, \*y, \*c, \*z) = \prod_{n=1}^N p(\*x_n | \*z_n)p(y_n | \*z_n)p(\*c_n | \*z_n) p(\*z).
% \end{equation}
% Here, $\*c \in \mathbb{R}^k$ are the `concepts' where $k<h$. The likelihoods are given by
% \begin{equation}
% \begin{gathered}
%     p(\*x_n | \*z_n) = \normaldist{\*x_n}{\*\mu_{\theta_x}(\*z_n)}{\text{diag}\ \*\sigma_{\theta_x}^2(\*z_n)} \\
%     p(y_n | \*z_n) = \normaldist{\*x_n}{\mu_{\theta_y}(\*z_n)}{\sigma_{\theta_y}^2(\*z_n)} \\
%     p(\*c_n | \*z_n) = \prod_{i=1}^k \normaldist{c_{nk}}{z_{nk}}{\sigma_c^2}.
% \end{gathered}
% \end{equation}
% Note that $p(\*c_n | \*z_n) = p(\*c_n | \{z_{ni}\}_{i=1}^k)$---that is, $\*c_n$ is modelled by just $k<h$ dimensions of the latent variable $\*z_n$.

% \subsection{Predictions}
% We are interested in the predictive distributions
% \begin{equation}
% \label{eq:predictive_distributions}
% \begin{gathered}
%     p(y_* | \*x_*) = \int p(y_* | \*z_*) p(\*z_* | \*x_*) d\*z_* \\
%     p(\*c_* | \*x_*) = \int p(\*c_* | \*z_*) p(\*z_* | \*x_*) d\*z_*
% \end{gathered}
% \end{equation}
% both of which require the posterior distribution $p(\*z_* | \*x_*)$. This is intractable for general likelihoods---instead, we introduce the variational approximation $q(\*z) \approx p(\*z | \*x)$. Technically, we should find this approximation by maximising
% \begin{equation}
%     \elbo = \expectargs{q(\*z)}{\log \frac{p(\*x | \*z)p(\*z)}{q(\*z)}}.
% \end{equation}
% However, this doesn't produce posterior distributions $q(\*z)$ which effectively model $\*y$ or $\*c$. Instead, we shall use the variational approximation $q(\*z) \approx p(\*z | \*x, \*y, \*c) \approx p(\*z | \*x)$ which can be found by maximising
% \begin{equation}
% \begin{aligned}
%     \elbo &= \expectargs{q(\*z)}{\log \frac{p(\*x | \*z)p(\*y | \*z)p(\*c | \*z)p(\*z)}{q(\*z)}} \\
%     &= \sum_{n=1}^N\left\{ \expectargs{q(\*z_n)}{\log p(\*x_n|\*z_n)p(y_n | \*z_n)p(\*c_n | \*z_n)} \right. \\
%     &\phantom{=\sum_{n=1}^N \{} \left. - \kl{q(\*z_n)}{p(\*z_n)} \right\}.
% \end{aligned}
% \end{equation}
% Since we expect the input $\*x_n$ to contain all the information contained in $\*c_n$ and $y_n$, we are justified in conditioning the parameters of $q(\*z_n)$ on $\*x_n$ alone:
% \begin{equation}
%     q(\*z_n) = \normaldist{\*z_n}{\*\mu_{\phi}(\*x_n)}{\Sigma_{\phi}(\*x_n)}.
% \end{equation}
% Replacing the true posterior in \eqref{eq:predictive_distributions} with the approximate posterior $q(\*z)$ gives the approximate predictive distributions
% \begin{equation}
% \begin{gathered}
%     p(y_* | \*x_*) \approx \int p(y_* | \*z_*) q(\*z_*) d\*z_* \\
%     p(\*c_* | \*x_*) \approx \int p(\*c_* | \*z_*) q(\*z_*) d\*z_*.
% \end{gathered}
% \end{equation}

% As discussed, one way to promote diversification is through the prior distribution $p(\*z)$. An alternative approach is to introduce posterior regularisation, which influences the posterior distributions. This is achieved by including a regulariser $\mathcal{R}(q(\*z))$ in the ELBO:
% \begin{equation}
%     \tilde{\mathcal{L}}_{\textrm{ELBO}} = \elbo + \gamma \sum_{n=1}^N \mathcal{R}(q(\*z_n))
% \end{equation}
% where the hyperparameter $\gamma$ determines the degree to which the posterior is regularised. Whilst many regularisers are appropriate, a natural choice is to define $\mathcal{R}(q(\*z_n))$ as
% \begin{equation}
% \small
% \begin{aligned}
%     \mathcal{R}(q&(\*z_n)) = \frac{1}{h(h-1)}\sum_{i=1}^h\sum_{j\neq i}^h \theta_{ij} \\
%     &-  \frac{\gamma}{d(d-1)}\sum_{i=1}^h\sum_{j\neq i}^h \left(\theta_{ij} - \frac{1}{d(d-1)} \sum_{p=1}^d\sum_{q\neq p}^d \theta_{pq}\right)^2
% \end{aligned}
% \end{equation}
% where 
% \begin{equation}
%     \theta_{ij} = \operatorname{arccos}\left(\frac{\expectargs{}{\*a_{ni}}\expectargs{}{\*a_{nj}}}{\|\expectargs{}{\*a_{ni}}\|_2\|\expectargs{}{\*a_{nj}}\|_2}\right)
% \end{equation}
% is the non-obtuse angle measuring the dissimilarity between vector representations of $z_{ni}$ and $z_{nj}$, $\*a_{ni}$ and $\*a_{nj}$. \emph{How do we obtain vector representations of $z_{ni}$ and $z_{nj}$?}



\subsection{Optimally Regularized Concepts}
Consider the case in which the probability distribution over the input, $p(\*x)$, can be factorized as
\begin{equation}
    p(\*x) = \prod_{i} p(\*x^{(i)})
\end{equation}
where the set $\mathcal{S} = \{\*x^{(i)}\}_{i}$ contains non-overlapping subsets of the input dimensions. Suppose that the new and old concepts depend on non-overlapping set of subsets of $\mathcal{S}$, such that $p(\*z_{:k} | \*x) = p(\*z_{:k} | \mathcal{S}_{\text{old}})$ and $p(\*z_{k:} | \*x) = p(\*z_{k:} | \mathcal{S}_{\text{new}})$, where $\mathcal{S}_{\text{new}}\subset \mathcal{S}$ and $\mathcal{S}_{\text{old}} \subset \mathcal{S}$. We then have
\begin{equation}
\begin{aligned}
    p(\*z_{k:}, \*z_{:k}) &= \int p(\*z_{k:}, \*z{:k} | \*x) p(\*x) d\*x \\ 
    &= \int p(\*z_{k:} | \mathcal{S}_{\text{new}}) p(\*z_{:k} | \mathcal{S}_{\text{old}}) d\mathcal{S}_{\text{new}} d\mathcal{S}_{\text{old}} \\
    &= p(\*z_{k:})p(\*z_{:k})
\end{aligned}
\end{equation}
i.e.\ the $\*z_{k:}$ and $\*z_{:k}$ are independent. Both the mutual information $I(\*z_{:k}, \*z_{k:})$ and distance covariance are zero in this case.
